AMLB: an AutoML Benchmark

Comparing different AutoML frameworks is notoriously challenging and often done incorrectly. We introduce an open and extensible benchmark that follows best practices and avoids common mistakes when comparing AutoML frameworks. We conduct a thorough comparison of 9 well-known AutoML frameworks across 71 classification and 33 regression tasks. The differences between the AutoML frameworks are explored with a multi-faceted analysis, evaluating model accuracy, its trade-offs with inference time, and framework failures. We also use Bradley-Terry trees to discover subsets of tasks where the relative AutoML framework rankings differ. The benchmark comes with an open-source tool that integrates with many AutoML frameworks and automates the empirical evaluation process end-to-end: from framework installation and resource allocation to in-depth evaluation. The benchmark uses public data sets, can be easily extended with other AutoML frameworks and tasks, and has a website with up-to-date results.

==> checklist.tex <==
legend:
 [?] not verified
 [ ] todo
 [o] partially done (could potentially be submitted as is)
 [x] to done
 [-] Only applicable in revision

General

[ ]    Make sure your abstract reads well. It will be used to advertise your paper.
[o]    We recommend you use small caps for system names.
[x]    Order of paper: At the end of your paper, the order of sections should be: Acknowledgments, Appendices, then References.
[x]    Acknowledgments should be a unnumbered section. You can use the \acks{} command for this.
[x]    Appendix section number should be a letter (Should look like Appendix A. Title). You can use \appendix followed by regular \section command to format appendices

Title Area

[x]    Capitalization of paper title: In the title area, the paper title should be in title case. (First letter of each word capitalized except for little words like "and" and "or".)
[x]    Author contact addresses: These should be complete enough that mail sent to that address will reach them
[-]    Editor listed: Please include the name of the Action Editor who handled your submission in the \editor{} tag
[o]    Keyword: Please add keywords to your article using \begin{keywords} ... \end{keywords} after your abstract. They should not be capitalised, they should be separated by commas, and they should not have a period at the end.
[x]    Abstract: Do not delete the % at the end of \begin{abstract}% as it introduces an extra indent
[x]    Title should be split across two lines, only when it is too long for one line.

Headers and Footers
% open issue with the first page footer (it's too long)
[o]    Front page header: Use the \jmlrheading command to get a correct header and footer on the title page
[x]    Copyright notice, bottom of front page uses authors full names: In the \jmlrheading command, please use the full names of all authors
[o]    Running headers: Add running headers to your paper using the \ShortHeadings command. Please see the example paper on the web site for how to do this. (https://www.jmlr.org/format/sample.pdf)
[x]    Running headers: In the \ShortHeadings command, please capitalise the words in your paper title.
[x]    Running headers: In the author list in the \ShortHeadings command, please use "and" before the last author
[x]    Running headers: The ShortHeadings author list should have last names only, and should list all authors if possible. If you have many authors, "et al." is acceptable. % (barely) fits on one page=>I think we're good?

Section Headers

[x]    No unnumbered sections: We do not use \paragraph or \section*. We do not allow bold, unindented text to begin a paragraph that could be mistaken for a section header. If it looks like a section header it needs to be numbered like a section header, otherwise it needs to be formatted in some other way (e.g., by indentation, or by using italics instead of boldface).
[x]    Section numbering: All sections, subsections, subsubsubsections must be numbered. Please use \subsubsection instead of \subsubsection*, etc
[x]    Capitalization of Section headings: All section headings should be title case. (First letter of each word capitalized except for little words like "and" and "or".) This includes subsections, sub subsections, etc.
[x]    Section headers: There must be some text separating all section headers

[?] Tables and Figures

[x] Float placement: In general, floats should be at the top or bottom of the page (avoid using [h] option to \begin{figure}). 
[x] Check for pages that contain several floats and only 2-3 lines of text. These will be confusing for a reader, who is likely to miss the text. When this happens, please put the floats on a floats page ([p] specifier) instead.
[x]    Floats should also be placed as close as possible to the page at which they are first referenced. You should not, e.g., place all of the figures at the end of the paper.
[x]    Figures, tables should be centered
[x]    Captions should be underneath figures and tables
[x]    Captions NOT in italics, bold
[o]    Tables and figures should not overfill margins
[x]    Multiline captions should have a hanging indent, that is, subsequent lines of the caption should be indented, aligning with the first word of the caption rather than the word "Figure". Usually this problem is caused by one of the other packages that you have included. Sometimes changing the order of includes will fix this (try moving the jmlr2e include farther down).

[x] Footnotes

[x]    Footnote markers should follow punctuation
[x]    Footnotes should be complete sentences

[x] Misc

[x]    Dashes: When using dashes in text, please use --- instead of --, with no space before or after---like this. (no dashes present)
[x]    Data set: We use "data set" rather than "dataset". (currently done with find-replace)

[?] Citations

    Carefully read the section on citations in Instructions for Formatting JMLR Articles. A quick guideline is that the paper should still read correctly if all parenthesized text were omitted. Here are examples of BAD citations:
        "See (Ginsberg, 1994) for an analysis..." [Uses citation as a noun]
        "Drummond (Drummond, 1994) showed that..." [Should be "Drummond (1994)"]
        "...the best method (see the ERT test (Davis, 1995))..." [double parens, should be "...best method (see the ERT test, Davis, 1995)..."]
    Citations not nested in parenthesis. Parentheses should not occur within parentheses, even for citations. Within parentheses use \citealt or \citealp instead. Or you can use \citep[e.g.,][]{smith00}.

[x] Object References

    Use \url commands to reference urls in papers. This causes hyperref to make the hyperlinks work nicely
    Parenthesis: \eqref can sometimes result in parentheses within parentheses. When referencing an equation within a parenthetical statement, use Equation 1 rather than (1) or Equation (1).
    When referencing figures, sections, etc. ("Figure 1", "Section 2.1"), please make sure the words "Figure", "Section", etc., are uppercase

[-] Math

    Punctuation: Math in formal writing should be punctuated as if the extra space is not there, for example, displayed equations should usually be followed by a comma or a period, depending on the surrounding text.
    Punctuation: Before displayed equations, punctuation (e.g., ":") is not necessary unless you would use the same punctuation if the equation were not there.
    In general, only equations that are referenced should be numbered. We are willing to relax this for equations that are particularly important, as others may wish to discuss these in later correspondence.
    Proofs should end with a filled box.
    Equations should not run over the right hand margin. Appendices are especially prone to this.
    Theorems, Lemmas, etc., should be labeled like Theorem 1, Theorem 2, Theorem 3, not as Theorem 2.1, Theorem 2.2, Theorem 2.3

[?] References

[ ]    It is preferable to cite published papers, rather than tech reports.
[ ]    Author names: Make citations consistent. Either give the full first name of all cited authors, or give the first initials only for all cited authors.
[ ]    Capitalization in paper titles: Titles of conference papers should have the first word only titles. However, watch out for words like Bayes and Markov. These should still be capitalized, but BibTeX often leaves uncapitalised incorrectly.
[ ]    Capitalization of book titles, etc: The parts in italics (book names, journal names, conf names) should be title case. (First letter of each word capitalized except for little words like "and" and "or".)
[ ]    Please cite conference titles consistently. We do not have a enforced style for conference names, but whichever style you choose, be consistent. Don't refer to the same conference as "AAAI 2004" in one reference and the "The Nineteenth National Conference on Artificial Intelligence" in another one. Personally, I prefer the style "International Conference on Machine Learning (ICML)", leaving off the "Proceedings of the Twentieth..."

From https://www.jmlr.org/format/format.html:

[ ] Scientists seem to like to use the Latin abbreviations i.e. and e.g. First, I'd like to encourage you to try to do without them. If you can't, then use the English equivalents (``that is'' instead of i.e. and ``for example'' instead of e.g.) If you really love the Latin (then you're a Latin lover?) you should at least do it right. There should be a period after each letter (because they're abbreviations), and there should be a comma after the expression.
